Dual-Pool Token-Budget Routing for Cost-Efficient and Reliable LLM Serving

Production vLLM fleets typically provision each instance for the worst-case context length, leading to substantial KV-cache over-allocation and under-utilized concurrency. In practice, 80-95% of requests are short, yet are served under configurations optimized for long contexts, wasting 4-8$\times$ throughput capacity and triggering reliability issues such as OOM crashes, preemption, and request rejections. We identify a common root cause for these inefficiencies: configuration-traffic mismatch. We propose dual-pool token-budget routing, a lightweight dispatch mechanism that partitions a homogeneous fleet into two specialized pools: a high-throughput short-context pool and a high-capacity long-context pool. Each request is routed based on its estimated total token budget, computed using a per-category bytes-to-token ratio that is learned online via exponential moving average from usage.prompt_tokens feedback, eliminating the need for a tokenizer. We also develop a simple analytical model that predicts fleet-level cost savings from workload characteristics and measured throughput differences, enabling practitioners to estimate benefits prior to deployment. Evaluations on real-world traces from the Azure LLM Inference Dataset and LMSYS-Chat-1M, serving Llama-3-70B on A100 GPUs, show that our approach reduces GPU-hours by 31-42%, corresponding to \$2.86M annual savings at fleet scale, while lowering preemption rates by 5.4$\times$ and improving P99 TTFT by 6%. A case study with Qwen3-235B-A22B on AMD MI300X at 10,000 req/s projects \$15.4M in annual savings. The method incurs only O(1) dispatch overhead, adapts automatically to heterogeneous workloads, and composes seamlessly with existing optimizations such as PagedAttention, continuous batching, and prefill-decode disaggregation.

==> Makefile <==
TEX      = pdflatex
BIBTEX   = bibtex
MAIN     = paper
PDF      = $(MAIN).pdf

.PHONY: all clean distclean watch

all: $(PDF)

$(PDF): $(MAIN).tex
	$(TEX) $(MAIN)
	$(TEX) $(MAIN)

clean:
	rm -f $(MAIN).aux $(MAIN).log $(MAIN).out $(MAIN).toc \
	      $(MAIN).bbl $(MAIN).blg $(MAIN).nav $(MAIN).snm \
	      $(MAIN).fdb_latexmk $(MAIN).fls $(MAIN).synctex.gz

distclean: clean
	rm -f $(PDF)

watch:
	@echo "Watching for changes..."
	@while true; do \
		inotifywait -q -e modify $(MAIN).tex && make all; \
	done

